What Makes a Scene ? Scene Graph-based Evaluation and Feedback for Controllable Generation

While text-to-image generation has been extensively studied, generating images from scene graphs remains relatively underexplored, primarily due to challenges in accurately modeling spatial relationships and object interactions. To fill this gap, we introduce Scene-Bench, a comprehensive benchmark designed to evaluate and enhance the factual consistency in generating natural scenes. Scene-Bench comprises MegaSG, a large-scale dataset of one million images annotated with scene graphs, facilitating the training and fair comparison of models across diverse and complex scenes. Additionally, we propose SGScore, a novel evaluation metric that leverages chain-of-thought reasoning capabilities of multimodal large language models (LLMs) to assess both object presence and relationship accuracy, offering a more effective measure of factual consistency than traditional metrics like FID and CLIPScore. Building upon this evaluation framework, we develop a scene graph feedback pipeline that iteratively refines generated images by identifying and correcting discrepancies between the scene graph and the image. Extensive experiments demonstrate that Scene-Bench provides a more comprehensive and effective evaluation framework compared to existing benchmarks, particularly for complex scene generation. Furthermore, our feedback strategy significantly enhances the factual consistency of image generation models, advancing the field of controllable image generation.

==> tables/algo_feedback.tex <==
\begin{algorithm}[t]
\caption{Scene Graph Feedback}\label{alg:feedback}
\textbf{Input:} Scene Graph $G = (V, E)$, Diffusion Model $f_{D}$, multimodal LLM $f_{M}$, LLM $f_L$ (can be $f_M$) \\ 
\textbf{Output:} Image $I_{\text{G}}$
\begin{algorithmic}[1]
\State $prompt \gets f_L(G)$ \Comment{Scene Composition}
\State $I_0 \gets f_{D}(prompt)$ \Comment{Generate initial image}
\State $V_{\text{pred}}, E_{\text{pred}} \gets f_{M}(I_0, G)$ \Comment{Evaluate objects and relationships}
\State $V_{\text{miss}} \gets V \setminus V_{\text{pred}}$ \Comment{Identify missing objects}
\State $E_{\text{miss}} \gets E \setminus E_{\text{pred}}$ \Comment{Identify missing relationships}
\State $G_{\text{miss}} \gets (V_{\text{miss}}, E_{\text{miss}})$ \Comment{Construct missing graph}
\If{$G_{\text{miss}} \neq (\emptyset, \emptyset)$} \Comment{If discrepancies exist}
    \State $prompt_{\text{miss}} \gets f_L(G_{\text{miss}})$
    \State $I_1 \gets f_D(prompt_{\text{miss}})$ \Comment{Generate reference image}
    \State $I_{\text{G}} \gets f_D(prompt, I_0, I_1)$ \Comment{Generate output using references}
\Else
    \State $I_{\text{G}} \gets I_0$
\EndIf
\State \Return $I_{\text{G}}$
\end{algorithmic}
\end{algorithm}
